A no-go theorem for Quantum theory ontological models

In this paper, we show that Quantum Mechanics does not admit ontological models, in the sense that the quantum state of a system cannot correspond to a set of physical states representing the independent reality of the system. We show, via two thought experiments based on the Wigner's friend scenario, that if the ontic state of physical systems in the lab is the same for Wigner and for his friend, one of the following will be violated: PBR theorem, Quantum-theoretic predictions, and the "No-superdeterminism" assumption.

==> mybibliography.tex <==
@incollection{wigner1995remarks,
  title={Remarks on the mind-body question},
  author={Wigner, Eugene P},
  booktitle={Philosophical reflections and syntheses},
  pages={247--260},
  year={1995},
  publisher={Springer}
}

@article{bell1964einstein,
  title={On the einstein podolsky rosen paradox},
  author={Bell, John S},
  journal={Physics Physique Fizika},
  volume={1},
  number={3},
  pages={195},
  year={1964},
  publisher={APS}
}

@incollection{kochen1975problem,
  title={The problem of hidden variables in quantum mechanics},
  author={Kochen, Simon and Specker, Ernst P},
  booktitle={The logico-algebraic approach to quantum mechanics},
  pages={293--328},
  year={1975},
  publisher={Springer}
}

@article{pusey2012reality,
  title={On the reality of the quantum state},
  author={Pusey, Matthew F and Barrett, Jonathan and Rudolph, Terry},
  journal={Nature Physics},
  volume={8},
  number={6},
  pages={475--478},
  year={2012},
  publisher={Nature Publishing Group}
}

@article{leifer2014quantum,
  title={Is the Quantum State Real? An Extended Review of $\psi$-ontology Theorems},
  author={Leifer, Matthew Saul},
  journal={Quanta},
  volume={3},
  number={1},
  pages={67--155},
  year={2014}
}

@incollection{brukner2017quantum,
  title={On the quantum measurement problem},
  author={Brukner, {\v{C}}aslav},
  booktitle={Quantum [Un] Speakables II},
  pages={95--117},
  year={2017},
  publisher={Springer}
}

@article{frauchiger2018quantum,
  title={Quantum theory cannot consistently describe the use of itself},
  author={Frauchiger, Daniela and Renner, Renato},
  journal={Nature communications},
  volume={9},
  number={1},
  pages={1--10},
  year={2018},
  publisher={Nature Publishing Group}
}

@article{barrett2014no,
  title={No $\psi$-epistemic model can fully explain the indistinguishability of quantum states},
  author={Barrett, Jonathan and Cavalcanti, Eric G and Lal, Raymond and Maroney, Owen JE},
  journal={Physical review letters},
  volume={112},
  number={25},
  pages={250403},
  year={2014},
  publisher={APS}
}

@article{bong2020strong,
  title={A strong no-go theorem on the Wigner’s friend paradox},
  author={Bong, Kok-Wei and et al.},
  journal={Nature Physics},
  pages={1--7},
  year={2020},
  publisher={Nature Publishing Group}
}

@article{laudisa2002relational,
  title={Relational quantum mechanics},
  author={Laudisa, Federico and Rovelli, Carlo},
  journal={The {Stanford} Encyclopedia of Philosophy},
  Note="\url{https://seop.illc.uva.nl/entries/qm-relational/}",
  year={2019}
}

@book{bell2004speakable,
  title={Speakable and unspeakable in quantum mechanics: Collected papers on quantum philosophy},
  author={Bell, John S and Bell, John Stewart},
  year={2004},
  publisher={Cambridge university press}
}

@misc{nielsen2002quantum,
  title={Quantum computation and quantum information},
  author={Nielsen, Michael A and Chuang, Isaac},
  year={2002},
  publisher={American Association of Physics Teachers}
}

@article{shimony1984contextual,
  title={Contextual hidden variables theories and Bell's inequalities},
  author={Shimony, Abner},
  journal={The British Journal for the Philosophy of Science},
  volume={35},
  number={1},
  pages={25--45},
  year={1984},
  publisher={Oxford University Press}
}

@incollection{fuchs2017participatory,
  title={On participatory realism},
  author={Fuchs, Christopher A},
  booktitle={Information and interaction},
  pages={113--134},
  year={2017},
  publisher={Springer}
}

@article{fuchs2017notwithstanding,
  title={Notwithstanding Bohr, the reasons for QBism},
  author={Fuchs, Christopher A},
  journal={Mind and Matter},
  volume={15},
  number={2},
  pages={245--300},
  year={2017},
  publisher={Imprint Academic}
}

@article{harrigan2010einstein,
  title={Einstein, incompleteness, and the epistemic view of quantum states},
  author={Harrigan, Nicholas and Spekkens, Robert W},
  journal={Foundations of Physics},
  volume={40},
  number={2},
  pages={125--157},
  year={2010},
  publisher={Springer}
}

@article{brukner2018no,
  title={A no-go theorem for observer-independent facts},
  author={Brukner, {\v{C}}aslav},
  journal={Entropy},
  volume={20},
  number={5},
  pages={350},
  year={2018},
  publisher={Multidisciplinary Digital Publishing Institute}
}

@article{price2008toy,
  title={Toy models for retrocausality},
  author={Price, Huw},
  journal={Studies in History and Philosophy of Science Part B: Studies in History and Philosophy of Modern Physics},
  volume={39},
  number={4},
  pages={752--761},
  year={2008},
  publisher={Elsevier}
}

@article{hooft2007free,
  title={The free-will postulate in quantum mechanics},
  author={Hooft, Gerard't},
  journal={arXiv preprint quant-ph/0701097},
  year={2007}
}

@article{barrett2018everett,
  title={Everett’s Relative-State Formulation of Quantum Mechanics},
  author={Barrett, Jeffrey},
  journal={The {Stanford} Encyclopedia of Philosophy},
  Note="\url{https://plato.stanford.edu/archives/win2018/entries/qm-everett/}",
  year={2018}
}

@article{Ghirardi2020collapse,
  title={Collapse Theories},
  author={Ghirardi, Giancarlo and Bassi, Angelo},
  journal={The {Stanford} Encyclopedia of Philosophy},
  Note="\url{https://plato.stanford.edu/archives/sum2020/entries/qm-collapse/}",
  year={2020}
}


@article{schlosshauer2005decoherence,
  title={Decoherence, the measurement problem, and interpretations of quantum mechanics},
  author={Schlosshauer, Maximilian},
  journal={Reviews of Modern physics},
  volume={76},
  number={4},
  pages={1267},
  year={2005},
  publisher={APS}
}

@article{ballentine1970statistical,
  title={The statistical interpretation of quantum mechanics},
  author={Ballentine, Leslie E},
  journal={Reviews of Modern Physics},
  volume={42},
  number={4},
  pages={358},
  year={1970},
  publisher={APS}
}

==> sections/acknowledgements.tex <==
\section*{Acknowledgements} \label{sec:acknowledgements}
    
